Microbiome Intervention Analysis with Transfer Functions and Mirror Statistics

Microbiome interventions provide valuable data about microbial ecosystem structure and dynamics. Despite their ubiquity in microbiome research, few rigorous data analysis approaches are available. In this study, we extend transfer function-based intervention analysis to the microbiome setting, drawing from advances in statistical learning and selective inference. Our proposal supports the simulation of hypothetical intervention trajectories and False Discovery Rate-guaranteed selection of significantly perturbed taxa. We explore the properties of our approach through simulation and re-analyze three contrasting microbiome studies. An R package, mbtransfer, is available at https://go.wisc.edu/crj6k6. Notebooks to reproduce the simulation and case studies can be found at https://go.wisc.edu/dxuibh and https://go.wisc.edu/emxv33.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> purgatory.tex <==


\textbf{Abstract}

\begin{enumerate}
\item Opening [Setting + Characters]: The human microbiome is dynamic, and it is sensitive to external influences. This has been the source of many interesting longitudinal studies (infants, cancer, wildfires).
\item Conflict : Though a variety of longitudinal modeling methods have been proposed, few have systematically studied how to incorporate the effect of external perturbations.
\item Action
\begin{enumerate}
	\item We adapt a classical idea from time series analysis to support intervention modeling in microbiota data.
	\item We compare alternative normalization approaches and model formulations (using trees, sparsity) through simulation.
	\item We illustrate the most effective approaches through data case studies: birth, diet changes, cancer transplants.
\end{enumerate}
\item Resolution
\begin{enumerate}
    \item Have prepared an R package to support this type of analysis.
    \item Make it possible to reason more evolutionarily and observe how communities both drift randomly and respond to specific environmental shifts.
    \item Opens the door to more complex environmental inputs, not just pulse perturbations.
\end{enumerate}
\end{enumerate}

\textbf{Introduction}

\begin{enumerate}
\item Motivating Figures
    \begin{enumerate}
	\item Show example changes in composition from the three studies we consider later on.
        \begin{enumerate}
		\item Give examples of specific questions we might ask of these data.
		\item Which taxa are most strongly affected by the intervention? Are the effects immediate or delayed? Are they short or long-term?
		\item We may expect differential responses according to particular environmental / subject conditions. What factors promote one dynamic response over another?
		\item After the intervention, does the community return to the same state as it started, does it shift to a new equilibrium, or does it never find an equilibrium?
        \end{enumerate}
	\item Describe their context and why they matter.
        \begin{enumerate}
		\item These data / questions give a glimpse into microbiome dynamics, and this could be very important for maintaining human and ecological health.
		\item We might be able to design interventions with specific long-run outcomes. Similarly, we may be able to identify factors that promote more resilient microbiomes.
        \end{enumerate}
    \end{enumerate}
\item Main Characters: Modeling Setting
        \begin{enumerate}
	\item Longitudinal data have received substantial attention in the statistical-methods-for-microbiome literature.
        \begin{enumerate}
		\item Generalized Lotka Volterra, MALLARD, Shenhav papers, MITRE, MDSINE, Dynamic Bayesian Networks.
		\item Some focus on classifying between outcome states (e.g., preterm vs. term). Many consider one-step ahead linear modeling (GLV, MALLARD, MDSINE).
        \end{enumerate}
        \end{enumerate}
\item Gap and why it matters
    \begin{enumerate}
	\item First, all these papers only consider immediate (one-step) effects, and if you want to model a delayed effect, you need an order Q autoregression.
	\item Second, though several papers mention you can include covariates, this never seems to have been explicitly implemented or discussed. 
        \begin{enumerate}
		\item The specific formulation can matter.
		\item Moreover, the differential dynamics and short vs. long-term effects questions were never considered.
        \end{enumerate}
    \end{enumerate}
\item Proposed approach
    \begin{enumerate}
	\item We will adapt the transfer function methodology of Box and Tiao. This allows systematic model building to account for delayed, long-term, and differential effects. There are a few difficulties, however,
        \begin{enumerate}
		\item Our time series are high-dimensional
		\item The data are count valued and confounded with total read depth. Using compositional and normalization methods is key.
		\item We have an entire collection of time series, one per environment / subject.
        \end{enumerate}
	\item How we get around those difficulties: consider several normalization and modeling variations of the original transfer function methodology.
        \begin{enumerate}
		\item We use the vector autoregressive analog of the original transfer function models,
              \begin{enumerate}
			\item We consider several forms of normalization (none, DESeq2 size factors, and MBImpute).
			\item We compare several model forms: Gaussian factor, Negative Binomial factor, and Tree-based.
              \end{enumerate}
		\item To understand differential dynamics
              \begin{enumerate}
			\item We add interaction terms between coefficients and conditions that might lead to different effects
			\item We consider regressing separately fitted (and smoothed) coefficients onto conditions.
              \end{enumerate}
		\item To understand short vs. long-term effects, we show how to construct impulse-response functions from the fitted models (testing is out of scope though…)
        \end{enumerate}
	\item Evaluation strategies
        \begin{enumerate}
		\item We use simulations with autoregressive negative binomial factor models. Gives a notion of sensitivity to normalization / modeling assumptions.
		\item We compute the post-intervention, k-step ahead prediction error. This allows us to see how well we predict short and long-run intervention effects. We compare against available packages for longitudinal modeling. We expect these to do poorly because they have no knowledge of the actual intervention timepoints.
		\item We use a variant of this simulation to evaluate detection of differential responses.
		\item Finally, consider evaluation with real data analysis case studies. We focus on ability to detect delayed effects, long-term shifts, and differential response.
        \end{enumerate}
    \end{enumerate}
\item Outline the rest of the paper
\end{enumerate}

These are notes about the potential data analysis. For each, we need to explain the high-level motivation
for studying the problem in the first place. Then we discuss the data that were collected and how they are
relevant to the overall question. We can discuss what a more naive statistical model would do, and we 
should give common-sense reasons for why they might not actually be optimal. Finally, we can go into the
transfer function approach and discuss how to practically implement it.
	
\section{Microbiome and Diet}

\begin{enumerate}
	\item In the early 1900's, Elie Metchnikoff became curious about how ingesting live bacteria might affect his health (partly because he was interested in longevity and aging). He began experimenting with himself, eating yoghurt for a few days and seeing whether it affected his microbiome. He noticed changes on the days where he ate the yoghurt, but he observed that the effects were always transient. Any attempts to remodel the gut microbiome  (for example, to live longer) would require a bit more attention.
	\item Fast forward 100 years, and we are only beginning to carefully understand the relationship between diet and the gut microbiome. With the advent of 16S sequencing, we are no longer limited to culturable bacteria (like Metchnikoff was). We can look into how the entire community changes when we change our diet.
	\item This was the premise of the David diet study. The study had people change to either plant or meat-based diets for a few days in a row, profiling their gut microbiome all through the process.
	\item A more naive analysis would just... 
		\begin{enumerate}
			\item Baseline 1. We can imagine using the GP method of Silverman (the \texttt{basset} function in \texttt{fido}). We would fit the collection of GPs across individuals, with covariates for when they did and did not receive the intervention. We can rank the taxa by the difference between the perturbed and unperturbed fitted series; we may even be able to apply the knockoff idea to this setting as well.
			\item Our main concern with this method is that, though it can learn mean-shifts during the intervention periods, it may struggle to learn the types of impulse patterns that are natural in transfer function modeling. This is a consequence of the fact that GP regression is essentially a smoothing strategy -- it does not learn specific dynamic responses from multiple historical lags. It also requires the same smoothness level across all timepoints, and may oversmooth during periods of perturbation and undersmooth during periods of stability.
			\item We can improve on this by including impulse responses from transfer functions. They can have immediate, non-smooth intervention effects. The main downside we anticipate is that, conditional on covariates, we are assuming a kind of stationarity, while GPs can more easily model change across times. The second improvement is that we can give a kind of ranking with false discovery rate guarantees, rather than just an ordered list (with no cutoff).
			\item Baseline 2. We can run the MDSINE model. It is nice that it already supports multiple perturbations in its tutorials. We can use it both to forecast future series and to rank taxa according to the coefficients from the input series.
			\item One important limitation of MDSINE is that it is quite slow -- it is running a full MCMC with updates required for the Dirichlet Process. Second, it can only look one time lag into the past, so we expect it struggles with delayed effects. Third, it assumes sparsity in taxa interactions, but might not have very efficient pooling of information across similar taxa. Finally, though we can interpret the fitted coefficients associated with the perturbation, we don't really have any guarantees about whether the coefficient is large enough to be really non-null.
			\item Transfer functions most directly address issue 2. If we can guarantee an efficient training strategy, we can also deal with issue 1, but this depends on our final fitting / estimation method. For issue 3, we may or may not have better luck when using some sort of factor structure.
			\item Note: Comparing to both these baselines in each of the data analysis is a bit more involved than what is often expected in this research area. In principle, we could simply compare forecasting accuracy and taxa selection using a simulation study (and, we should probably still do that). On the other hand, once we have code for that simulation, it wouldn't be hard to run the same code on the real data. We could still look at ground truth forecasting accuracy from all three methods (as we vary the forecast horizon from $1$ to $H$). We wouldn't have ground truth for taxa selection, but we can argue that the more predictive model is more likely to yield more useful inferences as well.
		\end{enumerate}
	\item What are the kinds of outputs that we want to share?
	\begin{enumerate}
		\item For each species, we want to know (1) whether it is influenced by the intervention / input, and (2) how it is affected by the intervention. From a testing perspective, we might want a ranking of which taxa are the most strongly influenced by the intervention. E.g., a measure of the area between the two hypothetical outcomes. For (2) we may want the shape of the impulse response function, together with some low-dimensional summary of how the impulse responses are similar / different across taxa. For (1), we may also some sort of calibration. The idea is we should flag taxa affected by the intervention, and among those that are flagged, we should control the fraction of false positives. I can imagine a knockoffs-based framework for this...
		\item So, we can imagine three outputs. Does each have a figure?
		\item For each type of intervention (across diets, across antibiotics, ...) a list of ``significantly'' affected microbes, together with an estimate of how important that feature is. This can be accompanied by a figure showing the observed intervention response along with the knockoff simulated trajectories.
		\item A dimensionality reduction figure showing the different shapes of taxon-level intervention responses and how they are related to one another. For example, those with delayed responses should be in one part of the figure and those with immediate responses should be somewhere else. You can accomplish this by showing the archetypal intervention responses and placing individual taxa in between, depending on their mixed-membership coefficients.
		\item A basic boxplot showing the prediction performance of a few different methods. The point is that we only want to trust inferences on methods that are actually strongly predictive. We will have a few different normalizations. We will compare to the \texttt{basset} function in \texttt{fido} and also MDSINE, following their tutorial \href{https://github.com/gerberlab/MDSINE2_Paper/}{https://github.com/gerberlab/MDSINE2\_Paper/}.
	\end{enumerate}
\end{enumerate}
	

\section{Bone Marrow Transplants}

\begin{enumerate}
	\item Setting and problem. Bone marrow transplants are among the most drastic actions that can be taken to combat blood cancers like leukemia. Bone marrow is where blood cells are created, and when these cells are cancerous, it is possible to replace the marrow that generates them. However, the effects of the transplantation are not immediate, and it takes time for the blood system to recover, becoming at home in its new host. During this period, the patient is extremely vulnerable to bacterial infection, because white blood cells coordinate the immune response. For this reason, patients are often given extreme regimens of antibiotics in the period preceding and immediately following each bone transplantion.
	\item We would like to know how each antibiotic influences microbiome composition. Which species are more resistant to which antibiotic regimens? How quickly do the antibiotics act, and how long does the effect last? Some patients presumably respond to the intervention differently than others -- are there any generalizable rules we can use to anticipate a patient's response?
	\item Quantitative comparisons
	\begin{enumerate}
		\item Forecasting error $h$ steps into the future, after holding out the data for all time after the transplantation (day 0 relative to intervention) on a subset of test subjects. This gives us a sense of the predictive power of a model.
		\item Total runtime. Faster methods are easier to recommend in practice.
		\item Fraction of overlap in inferences across methods. Which taxa are recovered by one method but not that others? Analyzing the specific trajectories can tell us whether certain effects are more easily recovered with some methods vs. others.
	\end{enumerate}
	\item Expected qualitative outputs
	\begin{enumerate}
		\item A dimensionality reduction figure of the impulse response patterns across taxa and antibiotics.
		\item A faceted figure of the three most significant impulse response functions, together with randomly drawn samples that have similar impulse response functions.
		\item The analogous figure showing heterogeneity in impulse response functions. We can interpret this with a precision medicine story -- there may be some types of patients with more sensitive microbiomes than others.
	\end{enumerate}
\end{enumerate}

\section{Childbirth}

\begin{enumerate}
	\item Setting and problem. After childbirth, a mother's inflammatory response is known to go through dramatic changes. These changes can influence the microbiome, and if the microbiome enters a new state, there might be elevated risk for long-term inflammatory issues. Therefore, we would like to understand (1) the typical response of the microbiome to childbirth and (2) sources of heterogeneity in these responses.
	\item Quantitative comparisons. We can use the same as for the bone marrow transplantation problem, except this time there is only one type of intervention of interest (childbirth).
	\item Expected qualitative outputs. This also feels quite similar to the previous part. We risk seeming redundant, but I also like the idea of including multiple related examples, just so people can see the generalizability of our ideas.
\end{enumerate}

\begin{enumerate}
	\item Some other examples we could consider: The gentamycin / high-fat mouse dataset from the MDSINE tutorials. The \texttt{mallard} bioreactor dataset available in the \texttt{fido} package.
\end{enumerate}

\end{document}

